DoubleU-Net: A Deep Convolutional Neural Network for Medical Image Segmentation

Semantic image segmentation is the process of labeling each pixel of an image with its corresponding class. An encoder-decoder based approach, like U-Net and its variants, is a popular strategy for solving medical image segmentation tasks. To improve the performance of U-Net on various segmentation tasks, we propose a novel architecture called DoubleU-Net, which is a combination of two U-Net architectures stacked on top of each other. The first U-Net uses a pre-trained VGG-19 as the encoder, which has already learned features from ImageNet and can be transferred to another task easily. To capture more semantic information efficiently, we added another U-Net at the bottom. We also adopt Atrous Spatial Pyramid Pooling (ASPP) to capture contextual information within the network. We have evaluated DoubleU-Net using four medical segmentation datasets, covering various imaging modalities such as colonoscopy, dermoscopy, and microscopy. Experiments on the MICCAI 2015 segmentation challenge, the CVC-ClinicDB, the 2018 Data Science Bowl challenge, and the Lesion boundary segmentation datasets demonstrate that the DoubleU-Net outperforms U-Net and the baseline models. Moreover, DoubleU-Net produces more accurate segmentation masks, especially in the case of the CVC-ClinicDB and MICCAI 2015 segmentation challenge datasets, which have challenging images such as smaller and flat polyps. These results show the improvement over the existing U-Net model. The encouraging results, produced on various medical image segmentation datasets, show that DoubleU-Net can be used as a strong baseline for both medical image segmentation and cross-dataset evaluation testing to measure the generalizability of Deep Learning (DL) models.

==> cutout.tex <==

\section{Abstract}
Automated polyp segmentation has Semantic segmentation is an important task in \ac{CADx} as it can provide meaningful information during surgery. This is the reason why \ac{ML}-based \ac{CADx} is gaining significant attention in clinical medicine. One of the major challenges in the field is to detect and track the position of the abnormalities during surgical procedures. To address this challenge, we provide the baselines experiment with the Kvasir-SEG dataset.  The proposed architecture can detect and segment multiple instances of the instrument at the same time. In practice, it is difficult to find annotated medical images with corresponding segmentation masks. In this paper, we present  Kvasir-SEG: an open-access dataset of gastrointestinal polyp images and corresponding segmentation masks, manually annotated by a medical doctor and then verified by an experienced gastroenterologist. Moreover, we also generated the bounding boxes of the polyp regions with the help of segmentation masks. We demonstrate the use of our dataset with advanced deep-learning based \ac{CNN} approach. The dataset and experiment will be the value for researchers to reproduce results and compare methods. Now, we enable multimedia and computer vision researchers to contribute in the field of polyp detection and automatic analysis of colonoscopy images.  The proposed method produced good results in terms of matrix like the dice coefficient, and \ac{mIoU}. Moreover, the proposed architecture has outperformed state of the art with CVC-612 dataset. 

%================================================================================
Among the primary health problem of contemporary society is cancer, with \ac{CRC} being the most prevailing strain globally ~\cite{haggar2009colorectal}. 
Early detection of \ac{CRC} is crucial for survival. Different research studies suggest that population-wide screening advances the prognosis and can even reduce the incidence of  \ac{CRC} \cite{holme2013flexible}. Current European Union guidelines ~\cite{von2012european} also recommend such screening for those above 50 years old.


Several methods exist for imaging the colorectal area, including conventional white-light endoscopy and virtual endoscopy~\cite{geetha2017heuristic}, and are readily available for gastroenterologists. Conventional white-light colonoscopy is regarded as the gold standard screening test for CRC~\cite{quintero2012progress}. Various randomized clinical examination and prospective cohort investigations have testified that conventional colonoscopy with polypectomy lowered the incidence of CRC significantly by 40-90 \% and decreased mortality~\cite{rex2002rationale}. Therefore, the requirement of colonoscopy continues to increase. \par
During colonoscopy, a very small video camera in the tip of the endoscope creates a video signal of the internal mucosa of the patients colon. The video data is shown on a monitor for real-time diagnosis by the endoscopist. Abnormalities such as polyps can be discovered and removed during the endoscopic procedure. 

Prior to the introduction of Wireless Capsule Endoscope (WCE), physicians could not examine the small intestine without any surgical operation. WCE was devised by a group of researchers in Baltimore in 1989, and afterwards introduced by Given Imaging Ltd., Yoqneam, Israel, as a commercial instrument. The device became publicly available in $2000$ and used wireless electronic technology~\cite{iddan2000wireless} that captures images of complete GI tract. This capsule-shaped pill can be shallowed by the patients in the presence of clinical experts without any discomfort~\cite{suman2017detection}. Unlike conventional endoscopy procedures, this procedure investigates the entire GIT without pain, sedation and air insufflation. WCE has assisted more than 1.6 million patients worldwide till now. An additional advantage of this new technology is the process of the physical examination that does not require the sedation and is non-invasiveness, so it only applies little pain to the patient~\cite{cui2010bleeding}. \par


Several conventional methods exist for colon examination. The most common among them are colonoscopy, CT colonography, and sigmoidoscopy. However, all of these procedures are time-consuming, expensive, and there is a possibility of side effects (for example, the risk of bleeding after colonoscopy).

A Segmentation of the surgical instruments is a challenging problem in robotics research. A robot-assisted system may require information for intra-operative guidance, which plays an essential role in decision making. This information may be images or videos that contain both instruments and information regarding patients intestinal tissue~\cite{shvets2018automatic}. Therefore, an accurate semantic segmentation would provide information regarding the presence of multiple instruments in the videos or images. Towards solving this task, We downloaded the dataset from Robust Medical Instrument Segmentation. 
The main contribution of the paper are as follows:
\begin{itemize}
   
\item We extend the Kvasir dataset~\cite{pogorelov2017kvasir} with polyp images along with their corresponding segmentation masks and bounding boxes. The \acp{ROI} are the pixels depicting polyp tissue. These are represented by a white foreground in the segmentation masks. The \acp{ROI} are generated from manual annotations verified by an experienced gastroenterologist. The bounding boxes are the set of coordinates that encloses the polyp regions. The Kvasir-SEG dataset is made publicly available and open access.

\item In this article, we include a first attempt to use the Kvasir-SEG dataset for pixel-wise semantic segmentation based analysis. For the experiment, we have used \ac{FCM}~\cite{CADx2007fast} and Deep Residual U-Net (ResUNet)~\cite{zhang2018road} architecture. We achieved promising results with our proposed methods when evaluated on the same dataset. We evaluated the proposed method using Dice Coefficients and mean \ac{IOU}. These metrics were selected for fair comparison, and we encourage the use of these and similar metrics in future work on the dataset. The promising results demonstrated in this paper serves as baseline and motivation for further research and evaluation done on the same dataset.

\item Multiple datasets are prerequisites for comparing computer vision based algorithms, and this dataset is useful both as a training dataset or as a validation dataset. This dataset can assist the development of state-of-the-art solutions on images captured by colonoscopes. Further research in this field has the potential to help reduce the polyp miss rate and thus improve examination quality. 
\end{itemize}


The paper is organized into five sections. Section~\ref{section:related_work} provides an overview of the related work in the field of automated \ac{GI} tract disease detection and polyp segmentation. In Section~\ref{section:resunetplusplus}, we describe the proposed architecture. Section~\ref{section:Experiment} describes the experiments. Section~\ref{section:Results} presents the results obtained from the experimental evaluation on different datasets. A discussion of the work is provided in Section~\ref{discussion}. Finally, we summarize the paper in Section~\ref{section:conclusion}.
%================================================================================
\section{Conclusion}
We proposed a novel architecture for the multi-instance instrument segmentation and multi-instance instrument detection task. The proposed method obtained promising results on the available dataset with dice coefficient of 0.999 and \ac{mIoU} of 0.447.

In future works, we plan to perform the same evaluation procedure to identify the generalizability of other \acf{ML} models such as regression, detection, and segmentation. Next, we will explore to what extent our trained networks can be reused for classifying different diseases in different datasets, with and without re-training. This opens wide range of research directions to identify more generalized models which are not biased to It is required to identify the cross-data generalization capacity of the datasets used in this experiments. Therefore, a simple classification model to classify datasets but not data labels will help researchers to identify the uniqueness of each dataset. This enables one of the future experiments and if these datasets are really unique to themselves, then researchers have to use multiple datasets for training to get a well-generalized model to use in practice.

%===============================================================================

\section{Related work}

Diakogiannis et al.~\cite{diakogiannis2020resunet} proposed ResUNet-a that is also an encoder-decoder based architecture like U-Net that uses residual connections, atrous convolution, pyramid scene parsing pooling and multitasking inference with a novel loss function based on dice loss. 






Many approaches exist for automatic polyp segmentation. Most of the prior polyp segmentation approaches are based on either polyp\textquotesingle s edge or texture whereas more recent ones used \ac{CNN} and pre-trained networks. Ganz et al.~\cite{ganz2012automatic} developed an extended tool, called Shape-UCM, that includes the prior knowledge about the shapes of polyps. This optical biopsy tool is used for automatically segmenting polyp on narrow-band imaging data. Yuan et al.~\cite{yuan2015improved} proposed an improved \ac{BoF} for the classification of the polyp in wireless capsule endoscopy images where they make use of the textural features from the neighboring pixel. Tajabakhsh et al.~\cite{tajbakhsh2015automated} designed a \ac{CADx} system that used hybrid context-shape approach for removing the non-polyp structure and shape information for localization of polyps. \par
Wang et al.~\cite{wang2016computer} designed a \ac{CADx} system that did not require human-specific annotations, and the system could automatically achieve online learning from weakly labeled data. Zhang et al.~\cite{zhang2016automatic} developed a fully automated system that could detect and differentiate hyperplastic and adenomatous colorectal polyp. Pozdeev et al.~\cite{pozdeev2019automatic} presented a fully automated polyp segmentation framework using pixel-wise prediction based upon the \ac{FCN}. One of the most completed related work is the polyp-detection system, i.e, a Polyp Alert ~\cite{wang2015polyp}, which has potential of providing a near real-time feedback during colonoscopy examination. Although the WCE has many advantages, further improvement of the technology is required. Currently, clinicians must inspect 50,000 and more images to locate the diseases which is a difficult task. They might miss the disease at an early stage due to visual fatigue or concentration loss.  While software developed by Given imaging exists that can detect active blood automatically, the sensitivity and specificity is very low. \par


There are several studies for the automatic detection of polyps. The most interesting studies among them are~\cite{mori2017computer,brandao2018towards,fernandez2016exploring,misawa2018artificial,wang2018development,bernal2017comparative,chen2018accurate,mori2018real,gkolfakis2017new,mori2018detecting,jha2019resunet++,wang2015polyp,thambawitacross2020,riegler2017annotation,yamada2019development}. One of the most recent and most complete work is by~\cite{wang2018development} — the model based on the deep learning algorithm, i.e., Segnet~\cite{badrinarayanan2017segnet} architecture.  The input dataset was collected from 1,290 patients that were used for training. Similarly, the dataset from 11,38 patients (27,113 colonoscopy images) was used for validation. They also trained the model using Segnet on the CVC-612 dataset and colonoscopy videos. They obtained high sensitivity, specificity, and receiver operating characteristics curve value. Their algorithm could achieve a speed of 25 frames per with some latency during real-time video analysis. The results suggest that the developed pipeline could be helpful to the endoscopists to differentiate between polyp and adenoma.\par
The above work is really interesting. However, one of the disadvantage of this work is that the dataset used in the study is not public. Additionally, the total number of images and videos used in the study are not sufficient enough to believe that the model is generalizable and could be useful in all the clinical trials. For, example, the model can predict with high sensitivity and precision on a certain dataset from one hospital and does not work on the dataset from the other hospital. One of the reason might be the types of imaging modality they used to capture videos or images during colonoscopy examination. Also, the study is retrospective. Therefore, we need to develop a robust support system that could potentially achieve high performances irrespective of the dataset. 

The summary of the related work shows that the automatic \ac{CADx} system for polyp detection/classification field is becoming more mature. Researchers are conducting study design from a retrospective study, prospective study, to post hoc examination of the prospectively obtained dataset. Also, the researchers are seen using imaging modalities such as white-light endoscopy, Magnifying NBI, Endocytoscopy, and their combinations for the experiments. The algorithm used for the design of the models is the ones that use handcrafted, \ac{CNN}, to pre-trained features from the ImageNet\cite{jha2019resunet++}. Additionally, the performance of the model is also seen to be improving. Moreover, some of the models are seen to be achieving very high performance. However, mostly they use small training and test datasets~\cite{brandao2018towards,wang2013part}. These current limitations make it harder to develop the generalizable system. Therefore, more efforts should be put toward developing the models by considering these challenges. In this paper, we attempt to develop a generalizable machine learning model for automatic polyp segmentation. 

%--------------------------------------------------------------------------------

%Polyp image segmentation can be challenging to the large variation in the size, shape, color, and structure of the polyp.

\subsection{Limitation of the study}
Why the systems can not be deployed in the hospitals yet?
\subsubsection{small data}
1. Transfer learning
2. Few-shot/one-shot learning
3. self-supervised learning
4. Data augmentation
\subsubsection{Robustness and Generalization}
1. Technical solutions
2. Start with human-in-the-loop

\subsubsection{Change management (Including safety/regulations}
